LibriheavyMix: A 20,000-Hour Dataset for Single-Channel Reverberant Multi-Talker Speech Separation, ASR and Speaker Diarization

The evolving speech processing landscape is increasingly focused on complex scenarios like meetings or cocktail parties with multiple simultaneous speakers and far-field conditions. Existing methodologies for addressing these challenges fall into two categories: multi-channel and single-channel solutions. Single-channel approaches, notable for their generality and convenience, do not require specific information about microphone arrays. This paper presents a large-scale far-field overlapping speech dataset, crafted to advance research in speech separation, recognition, and speaker diarization. This dataset is a critical resource for decoding ``Who said What and When'' in multi-talker, reverberant environments, a daunting challenge in the field. Additionally, we introduce a pipeline system encompassing speech separation, recognition, and diarization as a foundational benchmark. Evaluations on the WHAMR! dataset validate the broad applicability of the proposed data.

==> algo/_algo.tex <==
\begin{algorithm} 
	\caption{Data simulation} 
	\label{alg:simu} 
	\SetAlgoLined
    \KwData{$\mathcal{X}, \mathcal{M}, K, T$}
    \KwResult{$\mathcal{S}$} 
	$D_{={\rm spk}}, D_{\not={\rm spk}}, D_{\rm ovlp}, \mathcal{S} = \varnothing $ 
	
		\tcp{Fit the distribution of $\mathcal{M}$.}
		\ForEach{$m$ in $\mathcal{M}$} { 
		    \BlankLine
			\For{$i \leftarrow 1$ \KwTo $\operatorname{range}(|m|)$} {
				$t \leftarrow m_i.{\rm start} - m_{i-1}.{\rm end}$ 
				
				\eIf{$m_i.{\rm spk} == m_{i-1}.{\rm spk}$}{
					$D_{={\rm spk}} \leftarrow D_{={\rm spk}} \cup \{t\}$
				}{
					\lIf{$t > 0$} {$D_{\not={\rm spk}} \leftarrow D_{\not={\rm spk}} \cup \{t\}$}
					\lElse{$D_{\rm ovlp} \leftarrow D_{\rm ovlp} \cup \{-t\}$}
				}
			}
		}
		$P_{\rm ovlp}\leftarrow\frac{\left|D_{\rm ovlp}\right|}{\left|D_{\neq {\rm spk}}\right|+\left|D_{\mathrm{ovlp}}\right|}; $
		$D_* \leftarrow \operatorname{hist}\left(D_*\right)$
		
		\tcp{Generating mixtures using source utterances of $S$ speakers.}
		
		$\mathcal{X}=\left\{\mathcal{X}_1, \ldots, \mathcal{X}_S\right\}$
		
		\While {$\exists \mathcal{X}_s \in \mathcal{X} : |\mathcal{X}_s| > 0$ } {
			\tcp{Sample speakers.}
			$k \leftarrow {\rm sample}(K); \mathcal{X}_{s_1},\ldots, \mathcal{X}_{s_k} \leftarrow {\rm sample}(\mathcal{X})$
			
			\tcp{Sample utterances for each speaker.}
			\For{$i \leftarrow 1$ \KwTo $k$}{
				$U_{s_k} \leftarrow {\rm sample}\left(\mathcal{X}_{s_k}\right) \text {, s.t. }\left(\sum_{u \in U_{s_k}} u .{\rm dur}\right)<T $ 
				
				$\mathcal{X}_{s_k} \leftarrow \mathcal{X}_{s_k} \backslash U_{s_k} $
			}
			$U = {\rm shuffle}( U_{s_1}, \ldots,  U_{s_k})$
			
			${\rm offset} \leftarrow 0$
			
			\For{$i \leftarrow 1$ \KwTo ${\rm range}(|U|)$} {
				\eIf {$U_i$.{\rm spk} == $U_{i-1}$.{\rm spk}}{
					${\rm ot} = {\rm sample}(D_{={\rm spk}})$
				} {
					\lIf {{\it Bernoulli($P_{\rm ovlp} > 0.5$)}} {${\rm ot} = - {\rm sample}(D_{\rm ovlp})$}
					\lElse {${\rm ot} = {\rm sample}(D_{\not = {\rm spk}})$}
				}
				
				${\rm offset} = {\rm offset} + {\rm ot} $
				
				$\mathcal{S} = \mathcal{S} \cup \{U_i, {\rm offset}\}$
			}

		}
\end{algorithm}

==> sec/_1intro.tex <==
\section{Introduction}

Despite the rapid progress of automatic speech recognition (ASR) technologies \cite{wang2020transformer, gulati20_interspeech, yao2023zipformer} targeting near-field, non-overlap speech, accurate separation and recognition of overlapping speech remains a challenging task.
A wide range of research has been conducted to tackle the issue including, but not limited to mask estimation-based speech separation \cite{luo2018tasnet, luo2019conv}, permutation invariant training \cite{qian2018single, chang2019end, ZhangCQW20, meng2023sidecar}, transcript concatenation \cite{kanda20b_interspeech, kanda22_interspeech}, joint training of both front-end and backend systems \cite{von2020multi, raj2023surt}.
However, most of the existing approaches focus on the separation and recognition of near-field speech data, only limited research has been conducted targeting overlapped speech in reverberant conditions, which poses new challenges as reverberation causes spectral smearing of the source, causing further performance degradation of speech separation and recognition systems \cite{Maciejewski2020WHAMR, haeb2020far}.

Recently, scaling up the amount of training data has been proven to be critical on all fronts of speech-related tasks, including far-field multi-talker speech separation and recognition \cite{kadiouglu2020empirical, kanda2021large}.
However, the overlapping and reverberant condition of the task hinders the data collection process required for system pre-training and construction. 
Existing real-world far-field multi-talker datasets \cite{carletta2005ami, yu2022m2met} contain reverberation and multiple speaker turns, whereas these datasets are neither capable of speech separation construction due to the lack of clean source, nor capable of large-scale training due to limited amount of data and high costs associated with data recording and annotation.
This leads to a raising demand for in-domain, open-sourced datasets with large amounts of data for training and testing.

%these approaches and datasets \cite{panayotov2015librispeech,aishell_2017,kang2023libriheavy} can not handle the scenarios where multiple speakers speak simultaneously.

%Under the development of the speech community, researchers have proposed some simulated multi-talker overlapping speech datasets \cite{hershey2016deep,Wichern2019WHAM,Maciejewski2020WHAMR,cosentino2020librimix} to study speech separation \cite{hershey2016deep,YuKT017,luo2019conv,mossformer2} and multi-talker ASR \cite{yu2017recognizing,chang2019mimo,ZhangCQW20,kanda20b_interspeech,kanda22_interspeech}. However, most of these datasets do not take into account the reverberation in the far field, and the amount of data is not large enough. In addition, in these datasets, most of them are simple cases with less than 4 speaker turns, which does not match the multiple speaker turns of real-world conversational scenarios.

%In recent years, there are also some real-world recorded multi-speaker overlapping speech datasets \cite{carletta2005ami,yu2022m2met}, which naturally contain far-field reverberation and multiple speaker turns. However, the amount of these real-world recorded data is still not large enough due to the very high recording cost. Moreover, it is difficult to obtain clean separation targets from real-world recorded data, so it cannot be used for speech separation.

To this end, this work presents a 10,000-hour reverberant overlapped speech dataset LibriheavyMix derived from Libriheavy \cite{kang2023libriheavy}, which is a large-scale ASR corpus with richer information like punctuation casing and context.
Preliminary experiments on speech separation and multi-talker ASR were conducted on the proposed dataset. 
%The advantages of the proposed LibriheavyMix data is three folded. 
The contributions of this work are listed as follows:
{\bf (1)} The amount of training data delivered by LibriheavyMix outnumbered all previous overlapped speech datasets \cite{hershey2016deep, Wichern2019WHAM, cosentino2020librimix, Maciejewski2020WHAMR} as presented in Table \ref{tab:datasets}. 
{\bf (2)} A series of baseline systems are constructed and investigated on the proposed dataset. 
{\bf (3)} Further evaluation on previous public in-domain benchmark proves the proposed dataset is of significant generalizability for both separation and recognition tasks. 
{\bf (4)} Inherited from the simulation pipeline and Libriheavy dataset, the proposed dataset contains conversations with multiple speaker turns, speaker identity and accurate timestamp, along with casing, punctuation and text context, enabling the potential of various tasks such as speaker diarization \cite{park2022review, FujitaKHNW19, meng2023unified}, speaker-attributed ASR \cite{KandaYGWMCY21, YuDZL022, shi23d_interspeech} and systems with more flexibility.

%\begin{itemize}
%	\item[2)] Reverberation is introduced to simulate real-world far-field scenarios.
%    \item[3)] Multiple speaker turns, which is consistent with the real-world conversational scenarios, can be further used for speaker diarization \cite{park2022review,FujitaKHNW19,MedennikovKPKKS20,HeRHDC021} and speaker-attributed ASR \cite{KandaYGWMCY21, YuDZL022, shi23d_interspeech,ShiZDYCZD23}.
%    \item[4)] Punctuation casing and context is inherent in transcripts, which can be further combined with the research of punctuation and semantic information \cite{BijwadiaCLSZH22,shi23c_interspeech}.
%\end{itemize}

\input{tab/datasets}

The rest of this paper is organized as follows.
Section 2 presents the pipeline for data simulation. 
Section 3 describes the baseline systems for overlapped speech separation and recognition constructed on the proposed dataset. 
Section 4 shows experiments and results of baseline systems. 
Finally, Section 5 concludes this work.

% accurate separation and recognition of far-field overlapped speech remains a challenging task due to mixed signals from overlapping speakers and room reverberation. 
% These create a large mismatch between the reverberant mixture and dry clean speech. 


==> tab/cascaded.tex <==
\begin{table}[t]
  \caption{Performance of the cascaded systems on {\bf 2-speaker} test sets. Other naming conventions follow the one in Table \ref{tab:whamr_enh}.}
  \label{tab:cascaded}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c|c|c|c|c|c|c|c|c}
  	\toprule
  	\toprule
  	\multirow{3}{*}{Sys.} & \multicolumn{4}{c|}{Training Set} & \multicolumn{4}{c}{Word Error Rate (\%) $\downarrow$}    \\
	  & \multicolumn{3}{c|}{LibriheavyMix} & \multirow{2}{*}{WHAMR!} & \multirow{2}{*}{tt} & \multirow{2}{*}{dev} & \multirow{2}{*}{test-clean} & \multirow{2}{*}{test-other} \\
  	  & small & medium & large &  &  &  & \\
	\midrule
  	1 & \multicolumn{3}{c|}{-} & \checkmark &  &  &  &   \\
  	\midrule
  	2 & \checkmark &  &  & - &  & 95.8 &  &   \\
  	3 &  & \checkmark &  & - &  & 57.0 &  &   \\
  	4 &  &  & \checkmark & - &  & 34.8 &  &   \\
  	\midrule
  	5 & \checkmark &  &  & \checkmark &  &  &  &    \\
  	6 &  & \checkmark &  & \checkmark &  &  &  &   \\
   	7 &  &  & \checkmark & \checkmark &  &  &  &  \\
  	\bottomrule
  	\bottomrule
  \end{tabular}
  }
\end{table}

==> tab/conv_tasnet.tex <==
%\begin{table}[t]
%  \caption{Performance of the Conv-TasNet \cite{luo2019conv} models on the {\bf 2-speaker mixtures} subset of training and test data.}
%  \label{tab:conv_tasnet}
%  \centering
%  \resizebox{\linewidth}{!}{
%  \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
%  	\toprule
%  	\toprule
%  	\multirow{3}{*}{Sys.} & \multirow{3}{*}{\makecell[c]{Training \\ Set}} & \multicolumn{3}{c|}{SI-SDR $\uparrow$} & \multicolumn{3}{c|}{$\Delta$ SI-SDR $\uparrow$} & \multicolumn{3}{c}{Word Error Rate (\%) $\downarrow$} \\
%	  &  & \multirow{2}{*}{dev} & \multirow{2}{*}{\makecell[c]{test-\\clean}} & \multirow{2}{*}{\makecell[c]{test-\\other}} & \multirow{2}{*}{dev} & \multirow{2}{*}{\makecell[c]{test-\\clean}} & \multirow{2}{*}{\makecell[c]{test-\\other}} & \multirow{2}{*}{dev} & \multirow{2}{*}{\makecell[c]{test-\\clean}} & \multirow{2}{*}{\makecell[c]{test-\\clean}} \\
%  	  &  &  &  &  &  &  &  &  &  \\
%	\midrule
%  	1 & small & 6.16 & 7.57 & 5.93 & 7.08 & 7.65 & 6.12 & 88.9 & 93.9 & 94.1 \\
%  	2 & medium & 9.14 & 11.29 &	9.95 & 10.04 & 11.38 & 10.14 & 82.0 & 85.2 & 85.2  \\
%  	3 & large & 10.63 & 12.81 & 11.33 & 11.55 & 12.90 & 11.52 & 78.2 & 81.8 & 81.5 \\
%  	\bottomrule
%  	\bottomrule
%  \end{tabular}
%  }
%\end{table}

\begin{table}[t]
  \caption{Performance of the Conv-TasNet \cite{luo2019conv} models on the {\bf 2-speaker} training data and test sets of LibriheavyMix. ``dev'', ``test-clean'' and ``test-other'' denote the dev2spk, test-clean2spk and test-other2spk of LibriheavyMix.}
  \label{tab:conv_tasnet}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c|c|c|c|c|c|c|c}
  	\toprule
  	\toprule
  	\multirow{2}{*}{Sys.} & \multirow{2}{*}{\makecell[c]{Training  Set}} & \multicolumn{3}{c|}{SI-SDR $\uparrow$} & \multicolumn{3}{c}{$\Delta$ SI-SDR $\uparrow$} \\
	  &  & \multirow{1}{*}{dev} & \multirow{1}{*}{\makecell[c]{test-clean}} & \multirow{1}{*}{\makecell[c]{test-other}} & \multirow{1}{*}{dev} & \multirow{1}{*}{\makecell[c]{test-clean}} & \multirow{1}{*}{\makecell[c]{test-other}} \\
%  	  &  &  &  &  &  &  & \\
	\midrule
  	1 & {\it small2spk} & 6.16 & 7.57 & 5.93 & 7.08 & 7.65 & 6.12 \\
  	2 & {\it medium2spk} & 9.14 & 11.29 &	9.95 & 10.04 & 11.38 & 10.14 \\
  	3 & {\it large2spk} & 10.63 & 12.81 & 11.33 & 11.55 & 12.90 & 11.52  \\
  	\bottomrule
  	\bottomrule
  \end{tabular}
  }
\end{table}

==> tab/sot_2_mix.tex <==
\begin{table}[th]
  \caption{Performance of the Serialized Output Training (SOT) \cite{kanda20b_interspeech} AED models on training and test data of 2 speakers.}
  \label{tab:sot_aed_2_spkr}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c|c|c|c|c|c|c|c}
  	\toprule
  	\multirow{2}{*}{Sys.} & \multirow{2}{*}{\makecell[c]{Training \\ Set}} & \multicolumn{3}{c|}{Word Error Rate (\%)} & \multicolumn{3}{c}{Speaker Counting Acc (\%)} \\
	  &  & dev & test-clean & test-other & dev & test-clean & test-other \\
	\midrule
  	1 & small &  &  &  &  &  \\
  	2 & medium &  &  &  &  &  \\
  	3 & large &  &  &  &  &  \\
  	\bottomrule
  \end{tabular}
  }
\end{table}

==> tab/speakerbeam_2_mix.tex <==
\begin{table}[t]
  \caption{Performance of the SpeakerBeam \cite{vzmolikova2019speakerbeam} models on the {\bf 2-speaker mixtures} of training and test data.}
  \label{tab:speakerbeam_2_spkr}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
  	\toprule
  	\toprule
  	\multirow{3}{*}{Sys.} & \multirow{3}{*}{\makecell[c]{Training \\ Set}} & \multicolumn{3}{c|}{SI-SDR $\uparrow$} & \multicolumn{3}{c|}{$\Delta$ SI-SDR $\uparrow$} & \multicolumn{3}{c}{Word Error Rate (\%) $\downarrow$} \\
	  &  & \multirow{2}{*}{dev} & \multirow{2}{*}{\makecell[c]{test-\\clean}} & \multirow{2}{*}{\makecell[c]{test-\\other}} & \multirow{2}{*}{dev} & \multirow{2}{*}{\makecell[c]{test-\\clean}} & \multirow{2}{*}{\makecell[c]{test-\\other}} & \multirow{2}{*}{dev} & \multirow{2}{*}{\makecell[c]{test-\\clean}} & \multirow{2}{*}{\makecell[c]{test-\\clean}} \\
  	  &  &  &  &  &  &  &  &  &  \\
	\midrule
  	1 & small & 3.00 & 4.45 & 3.18 & 3.93 & 4.47 & 3.36 &  &  \\
  	2 & medium &  &  &  &  &  &  &  &  \\
  	3 & large &  &  &  &  &  &  &  &  \\
  	\bottomrule
  	\bottomrule
  \end{tabular}
  }
\end{table}

==> tab/speakerbeam_var_mix.tex <==
\begin{table}[th]
  \caption{Performance of the SpeakerBeam \cite{vzmolikova2019speakerbeam} models on various mixtures of training and test data.}
  \label{tab:speakerbeam_var_spkr}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c|c|c|c|c|c|c|c}
  	\toprule
  	\multirow{2}{*}{Sys.} & \multirow{2}{*}{\makecell[c]{Training \\ Set}} & \multicolumn{3}{c|}{SI-SNR} & \multicolumn{3}{c}{Word Error Rate (\%)} \\
	  &  & dev & test-clean & test-other & dev & test-clean & test-other \\
	\midrule
  	1 & small &  &  &  &  &  \\
  	2 & medium &  &  &  &  &  \\
  	3 & large &  &  &  &  &  \\
  	\bottomrule
  \end{tabular}
  }
\end{table}

